Symmetric Operations on Domains of Size at Most 4

To convert a fractional solution to an instance of a constraint satisfaction problem into a solution, a rounding scheme is needed, which can be described by a collection of symmetric operations with one of each arity. An intriguing possibility, raised in a recent paper by Carvalho and Krokhin, would imply that any clone of operations on a set $D$ which contains symmetric operations of arities $1, 2, \ldots, \lvert D \rvert$ contains symmetric operations of all arities in the clone. If true, then it is possible to check whether any given family of constraint satisfaction problems is solved by its linear programming relaxation. We characterize all idempotent clones containing symmetric operations of arities $1, 2, \ldots, \lvert D \rvert$ for all sets $D$ with size at most four and prove that each one contains symmetric operations of every arity, proving the conjecture above for $\lvert D \rvert \leq 4$.

==> temp.tex <==
% there's 3 versions, v2 is just a faster version of v1, and v3 is optimized for symmetric operations
% I write papers with "a version of me who hasn't learned this yet" as my intended audience
% in some cases, I write with "zhuk and his buddies" as an intended audience
% it really helps if you can imagine a particular person reading your paper
% and wondering what the heck you are doing
% how can I define "functional equation" with the fewest words necessary
% oh, do I want to say "idempotent round clone" or "round idempotent clone"
% FIX THE RPS INDUCTION
